Worse than Random? An Embarrassingly Simple Probing Evaluation of Large Multimodal Models in Medical VQA

Large Multimodal Models (LMMs) have shown remarkable progress in medical Visual Question Answering (Med-VQA), achieving high accuracy on existing benchmarks. However, their reliability under robust evaluation is questionable. This study reveals that when subjected to simple probing evaluation, state-of-the-art models perform worse than random guessing on medical diagnosis questions. To address this critical evaluation problem, we introduce the Probing Evaluation for Medical Diagnosis (ProbMed) dataset to rigorously assess LMM performance in medical imaging through probing evaluation and procedural diagnosis. Particularly, probing evaluation features pairing original questions with negation questions with hallucinated attributes, while procedural diagnosis requires reasoning across various diagnostic dimensions for each image, including modality recognition, organ identification, clinical findings, abnormalities, and positional grounding. Our evaluation reveals that top-performing models like GPT-4o, GPT-4V, and Gemini Pro perform worse than random guessing on specialized diagnostic questions, indicating significant limitations in handling fine-grained medical inquiries. Besides, models like LLaVA-Med struggle even with more general questions, and results from CheXagent demonstrate the transferability of expertise across different modalities of the same organ, showing that specialized domain knowledge is still crucial for improving performance. This study underscores the urgent need for more robust evaluation to ensure the reliability of LMMs in critical fields like medical diagnosis, and current LMMs are still far from applicable to those fields.

==> sections/tables/ablation_cot_som.tex <==
\begin{table}[t]
% \small
\caption{\textbf{Probing analysis on the affect of different prompting methods on MLLMs' performance. Performance under different probing settings is compared with the vanilla setting.} Gains are in blue and drops are in red.
}
\begin{center}
\vspace{-10pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule

Models & Vanilla & + CoT & + SoM & + Both & MM-CoT\\
\midrule
\multicolumn{6}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
o1 (1217)           & 51.40  & -- & \textcolor{red}{-0.66}  & -- & \textcolor{blue}{+0.09}\\
GPT-4o (1120)       & 33.14  & -- & \textcolor{blue}{+5.34} & -- & \textcolor{blue}{+4.40}\\
\multicolumn{6}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
Qwen2.5-VL-7B       & 17.60 & \textcolor{blue}{+0.28} & \textcolor{blue}{+0.09} & \textcolor{blue}{+0.28} &\\ 
LLaVA-NeXT-7B       & 14.70 & \textcolor{red}{-1.78}  & \textcolor{red}{-2.53} & \textcolor{red}{-0.47} & \\
InternVL2.5-8B      & 14.23 & \textcolor{blue}{+2.24} & \textcolor{red}{-0.66} & \textcolor{red}{-1.41} & \\
Phi-3.5-Vision-4B   & 14.23 & \textcolor{red}{-0.38}  & \textcolor{blue}{+0.47} & \textcolor{blue}{+0.84} & \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\label{tab:ablation_cot_som}
\end{table}


==> sections/tables/ablation_mmcot.tex <==
\begin{table}[t]
% \small
\caption{\textbf{Model performance after probing with MM-CoT.} Performance gain are in parentheses.}
\begin{center}
\vspace{-10pt}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lcc}
\toprule

Models & Vanilla & + MM-CoT \\
\midrule
\multicolumn{3}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
o1 (1217)           & 51.40  & 51.77 (\textcolor{blue}{+0.37})\\
GPT-4o (1120)       & 33.14  & 45.88 (\textcolor{blue}{+12.74})\\
\multicolumn{3}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
Qwen2.5-VL-7B       & 17.60  & 23.68  (\textcolor{blue}{+6.08})\\   
LLaVA-NeXT-7B       & 14.70  & 17.41  (\textcolor{blue}{+2.71})\\   
InternVL2.5-8B      & 14.23  & 15.26  (\textcolor{blue}{+1.02})\\ 
Phi-3.5-Vision-4B   & 14.23  & 14.23  (\textcolor{black}{+0.00})\\ 
\bottomrule
\end{tabular}
}
\end{center}
% \vspace{-10pt}
\label{tab:mmcot}
\end{table}


==> sections/tables/main_result.tex <==
\begin{table*}[t]
% \small
\caption{\textbf{The accuracy of six MLLMs under the two evaluation settings.} Proprietary models demonstrate higher performance as well as larger performance gain in the MCQ setting.}
\begin{center}
\vspace{-10pt}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcccc|cccc}
\toprule

& \multicolumn{4}{c}{\textbf{Open-ended}} & \multicolumn{4}{c}{\textbf{Multiple-choice}} \\
\cmidrule(l){2-5}
\cmidrule(l){6-9}

Models & Web & Office & Poster & Overall & Web & Office & Poster & Overall\\

\midrule
\multicolumn{9}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
o1 (1217)         & 47.91 & 59.19 & 38.73 & 51.40 & 47.91 & 58.52 & 46.47 & 52.15 \\
GPT-4o (1120)     & 25.00 & 42.60 & 30.98 & 33.14 & 37.29 & 58.96 & 47.88 & 47.75 \\
\multicolumn{9}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
Qwen2.5-VL-7B     & 8.54  & 29.14 & 11.97 & 17.60 & 14.37 & 33.18 & 16.90 & 22.56 \\  
LLaVA-NeXT-7B     & 10.20 & 21.97 & 7.04  & 14.70 & 11.45 & 25.33 & 5.63  & 16.47 \\
InternVL2.5-8B    & 7.70  & 24.21 & 4.92  & 14.23 & 9.37  & 23.54 & 11.97 & 15.63 \\
Phi-3.5-Vision-4B & 6.87  & 24.43 & 7.04  & 14.23 & 1.66  & 8.52  & 0.00  & 4.30  \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\label{tab:main_eval_result}
\end{table*}


% \begin{table}[t]
% % \small
% \caption{\textbf{We present the accuracy of six MLLMs under four different settings, each across three artifact types.}}
% \begin{center}
% \vspace{-10pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{clcccc}
% \toprule

% \multicolumn{1}{c}{} & Models & \textbf{Web} & \textbf{Office} & \textbf{Poster} & \textbf{Overall}\\

% \midrule
% \multirow{8}{*}{\rotatebox[origin=c]{90}{Open-ended}} 
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
% & o1 (1217)         & 47.91 & 59.19 & 38.73 & 51.40 \\
% & GPT-4o (1120)     & 25.00 & 42.60 & 30.98 & 33.14 \\
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
% & Qwen2.5-VL-7B     & 8.54  & 29.14 & 11.97 & 17.60 \\   
% & LLaVA-NeXT-7B     & 10.20 & 21.97 & 7.04  & 14.70 \\
% & InternVL2.5-8B    & 7.70  & 24.21 & 4.92  & 14.23 \\
% & Phi-3.5-Vision-4B & 6.87  & 24.43 & 7.04  & 14.23 \\

% \midrule
% \multirow{8}{*}{\rotatebox[origin=c]{90}{SoM-MCQ}} 
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
% & o1 (1217)         & 39.16 & 52.69 & 24.64 & 42.88 \\
% & GPT-4o (1120)     & 23.75 & 54.58 & 21.12 & 36.23 \\
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
% & Qwen2.5-VL-7B     & 2.91  & 28.02 & 4.92  & 13.67 \\   
% & LLaVA-NeXT-7B     & 0.41  & 19.95 & 6.33  & 9.36  \\
% & InternVL2.5-8B    & 2.70  & 21.74 & 4.22  & 10.86 \\
% & Phi-3.5-Vision-4B & 0.83  & 13.67 & 7.04  & 7.02  \\

% \midrule
% \multirow{8}{*}{\rotatebox[origin=c]{90}{Cap-MCQ}} 
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
% & o1 (1217)         & 47.91 & 58.52 & 46.47 & 52.15 \\
% & GPT-4o (1120)     & 37.29 & 58.96 & 47.88 & 47.75 \\
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
% & Qwen2.5-VL-7B     & 14.37 & 33.18 & 16.90 & 22.56 \\   
% & LLaVA-NeXT-7B     & 11.45 & 25.33 & 5.63  & 16.47 \\
% & InternVL2.5-8B    & 9.37  & 23.54 & 11.97 & 15.63 \\
% & Phi-3.5-Vision-4B & 1.66  & 8.52  & 0.00  & 4.30  \\

% \midrule
% \multirow{8}{*}{\rotatebox[origin=c]{90}{Cap-SoM-MCQ}} 
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Proprietary Models}}\\
% & o1 (1217)         & 48.33 & 55.38 & 44.36 & 50.74 \\
% & GPT-4o (1120)     & 39.58 & 56.50 & 47.18 & 47.65 \\
% & \multicolumn{5}{>{\columncolor{gray!15}}l}{\textit{Open-sourced Models}}\\
% & Qwen2.5-VL-7B     & 15.83 & 35.20 & 15.49 & 23.87 \\
% & LLaVA-NeXT-7B     & 11.45 & 24.88 & 7.04  & 16.47 \\
% & InternVL2.5-8B    & 8.33  & 26.23 & 14.78 & 16.66 \\
% & Phi-3.5-Vision-4B & 7.70  & 13.90 & 1.40  & 9.45  \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% % \vspace{-2em}
% \vspace{-10pt}
% \label{tab:main_eval_result}
% \end{table}


==> sections/tables/statistics.tex <==
\begin{table}[t]
\caption{\textbf{MMIR Statistics.} Breakdown of the dataset by artifact category and error type.}
\vspace{-10pt}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcr}
\toprule
\textbf{Category} & \textbf{\#Questions} & \textbf{Ave. \#Elements} \\
\midrule
\multicolumn{3}{l}{\textbf{Artifact Categories}} \\
\hspace{3mm} Web                & 240   & 38.8 \\
\hspace{6mm} - Shopping         & 108   & 46.1 \\
\hspace{6mm} - Wiki             & 28    & 44.9 \\
\hspace{6mm} - Classifieds      & 104   & 29.5 \\
\hspace{3mm} Office             & 223   & 9.1 \\
\hspace{6mm} - Slides           & 102   & 9.4 \\
\hspace{6mm} - Tables/Charts    & 61    & 4.1 \\
\hspace{6mm} - Diagrams         & 60    & 13.9 \\
\hspace{3mm} Poster             & 71    & 27.6 \\
\textbf{Total}                  & 543   & 24.9 \\

\midrule
\multicolumn{3}{l}{\textbf{Error Categories}} \\
\hspace{3mm} Factual Contradiction          & 138   & -- \\
\hspace{3mm} Identity Misattribution        & 84    & -- \\
\hspace{3mm} Contextual Mismatch            & 141   & -- \\
\hspace{3mm} Quantitative Discrepancy       & 76    & -- \\
\hspace{3mm} Temporal/Spatial Incoherence   & 95    & -- \\
\textbf{Total}                              & 543   & -- \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:statistics}
\end{table}
